Winning Strategies for the Synchronization Game on Subclasses of Finite Automata

We exhibit a winning strategy for Synchronizer in the synchronization game on every synchronizing automaton in whose transition monoid the regular D-classes form subsemigroups

==> eptcsdata.tex <==
\providecommand{\firstpage}{77}
\providecommand{\publicationstatus}{Giovanni Pighizzini, Florin Manea (Eds.): NCMA 2024\\
EPTCS 407, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.407.6}{10.4204/EPTCS.407.6}}
\pdfoutput=1

